Benefit of Self-Stabilizing Protocols in Eventually Consistent Key-Value Stores: A Case Study

In this paper, we focus on the implementation of distributed programs in using a key-value store where the state of the nodes is stored in a replicated and partitioned data store to improve performance and reliability. Applications of such algorithms occur in weather monitoring, social media, etc. We argue that these applications should be designed to be stabilizing so that they recover from an arbitrary state to a legitimate state. Specifically, if we use a stabilizing algorithm then we can work with more efficient implementations that provide eventual consistency rather than sequential consistency where the data store behaves as if there is just one copy of the data. We find that, although the use of eventual consistency results in consistency violation faults (cvf) where some node executes its action incorrectly because it relies on an older version of the data, the overall performance of the resulting protocol is better. We use experimental analysis to evaluate the expected improvement. We also identify other variations of stabilization that can provide additional guarantees in the presence of eventual consistency.Finally, we note that if the underlying algorithm is not stabilizing, even a single \cvf may cause the algorithm to fail completely thereby making it impossible to benefit from this approach.

==> old-intro.tex <==
As faults are inevitable in distributed systems, fault-tolerance is desirable for any reliable distributed algorithms. Fault tolerance can be either forward or backward. In the former case, we need a mechanism for detection of faults and another mechanism to rollback the system to a state before the faults happened. In the later case, the computation keeps running and when faults stop happening, any incorrect results caused by the faults will be eventually resolved by design of the algorithms itself. In particular, the algorithms contain transition that, when faults cease, bring systems from faulty states to non-faulty (or legitimate) states \cite{AG1993TSE,KA2000FTRTFT}. In this case, the algorithms are self-stabilizing. Self-stabilizing algorithms are desirable when faults happen in burst since in such scenarios, rolling back the system is costly since we have to roll back each time a fault occurs. The best case for the performance of self-stabilizing algorithms is when there is no fault, in which correct results are obtained fastest.

In this paper, we consider an approach to further improve the performance of self-stabilizing algorithms when they are run on key-value stores. Key-value stores are increasingly popular today due to their minimal structure for data and high performance \cite{DHJKLPSVV07SOSP,Voldemort}. Due to the implications of the CAP theorem \cite{Brewer00PODC,GL02SIGACT}, a distributed key-value store cannot achieve simultaneously three desirable properties: strong consistency (C), availability (A), and network partition tolerance (P). As network partition is considered a must today \todo{more explanation}, key-value store designers usually make the trade-offs between consistency and availability. As a result, a key-value store can run under a strong consistency model with low availability or under a weak consistency model (such as causal consistency \cite{DIRZ14SOCC,LFKA11SOSP,RDK17SRDS}, eventual consistency \cite{DHJKLPSVV07SOSP,LM10SIGOPS,Voldemort,SKGFSS12FAST}) with high availability.

When designing distributed algorithms, including self-stabilizing ones, on a key-value store, it is more natural for a algorithm designer to think that the store is strongly consistent, i.e. the key-value store acts as if it were a single store while in reality it consists of multiple distributed stores. That expectation relieves the designer of the data storage handling burden (e.g. data replication, making sure data consistent) and let him focus on the logic of the algorithms. Hence, in the ideal condition when the key-value store is strongly consistent and there is no fault, a self-stabilizing algorithm is expected to operate at its best performance. In this paper, we want to consider a possibility to further improve the performance of self-stabilizing algorithms in key-value stores by letting the algorithms run on a weaker consistency model such as eventual consistency.

When operating under the eventual consistency model, key-value stores provide higher throughput \cite{DHJKLPSVV07SOSP,NCKD2018TR} at the cost of possible data conflicts. As data conflicts happen, the self-stabilizing algorithms have to undergo the convergence process to correct the results, which slow down the algorithms progress. However, experiments suggest that such data conflicts are rare \cite{DHJKLPSVV07SOSP,NCKD2018TR}. Therefore, the slowdown due to fault-triggered convergence can be well compensated by the accelerated performance in eventual consistency model and in overall, the algorithms progress faster in eventual consistency.

In this paper, we examine this hypothesis by running some practical self-stabilizing algorithms on the Voldemort key-value store. We run our experiments on Amazon AWS ECS machines. From the experiments, we attain the following observations:
\begin{itemize}
\item Running a maximal matching self-stabilizing algorithm on eventual consistency progresses $XYZ\%$ faster than running on sequential consistency.
\item The number of fault-triggered convergences is $ABC$. On average, the cost of each convergence is $XYZ\ s$ \todo{We may need some monitoring mechanism to obtain this data}. 
\item We may compare how different algorithms for the same problem converge at different speed under a particular kind of fault.
It may be possible convergence of self-stabilizing algorithms for different problems have differently properties.
\end{itemize}

